The Touch\'e23-ValueEval Dataset for Identifying Human Values behind Arguments

We present the Touch\'e23-ValueEval Dataset for Identifying Human Values behind Arguments. To investigate approaches for the automated detection of human values behind arguments, we collected 9324 arguments from 6 diverse sources, covering religious texts, political discussions, free-text arguments, newspaper editorials, and online democracy platforms. Each argument was annotated by 3 crowdworkers for 54 values. The Touch\'e23-ValueEval dataset extends the Webis-ArgValues-22. In comparison to the previous dataset, the effectiveness of a 1-Baseline decreases, but that of an out-of-the-box BERT model increases. Therefore, though the classification difficulty increased as per the label distribution, the larger dataset allows for training better models.

==> table-bert-label-scores.tex <==
\begin{table*}
\setlength{\tabcolsep}{2pt}\centering
\footnotesize
\begin{tabular}{@{}l@{\hspace{6pt}}cccc@{\hspace{6pt}}cccc@{\hspace{6pt}}cccc@{\hspace{6pt}}cccc@{}}
\toprule
\bf Label & \multicolumn{4}{c}{\bf Africa} & \multicolumn{4}{c}{\bf China} & \multicolumn{4}{c}{\bf India} & \multicolumn{4}{c}{\bf USA}\\
\cmidrule(r{6pt}){2-5}
\cmidrule(r{6pt}){6-9}
\cmidrule(r{6pt}){10-13}
\cmidrule{14-17}
& \bf P & \bf R & \bf F$_1$ & \bf Acc & \bf P & \bf R & \bf F$_1$ & \bf Acc & \bf P & \bf R & \bf F$_1$ & \bf Acc & \bf P & \bf R & \bf F$_1$ & \bf Acc\\
\midrule
Be creative & - & - & - & - & 0.00 & 0.00 & 0.00 & 0.96 & 0.00 & 0.00 & 0.00 & 0.98 & 1.00 & 0.08 & 0.15 & 0.98 \\
Be curious & - & - & - & - & 0.50 & 0.33 & 0.40 & 0.97 & 0.00 & 0.00 & 0.00 & 0.98 & 0.29 & 0.11 & 0.15 & 0.96 \\
Have freedom of thought & 1.00 & 0.50 & 0.67 & 0.96 & - & - & - & - & 0.20 & 0.25 & 0.22 & 0.93 & 0.42 & 0.32 & 0.36 & 0.84 \\
Be choosing own goals & - & - & - & - & 0.33 & 0.33 & 0.33 & 0.96 & 0.33 & 0.25 & 0.29 & 0.95 & 0.74 & 0.34 & 0.46 & 0.84 \\
Be independent & 0.00 & 0.00 & 0.00 & 0.92 & 1.00 & 0.33 & 0.50 & 0.98 & - & - & - & - & 0.57 & 0.19 & 0.28 & 0.87 \\
Have freedom of action & 0.25 & 0.25 & 0.25 & 0.88 & 0.33 & 0.33 & 0.33 & 0.96 & 0.38 & 1.00 & 0.55 & 0.95 & 0.64 & 0.40 & 0.50 & 0.85 \\
Have privacy & - & - & - & - & 0.00 & 0.00 & 0.00 & 0.96 & 0.00 & 0.00 & 0.00 & 0.93 & 0.00 & 0.00 & 0.00 & 0.99 \\
Have an exciting life & - & - & - & - & - & - & - & - & 0.00 & 0.00 & 0.00 & 0.99 & 0.00 & 0.00 & 0.00 & 0.99 \\
Have a varied life & - & - & - & - & - & - & - & - & - & - & - & - & 0.00 & 0.00 & 0.00 & 0.95 \\
Be daring & - & - & - & - & - & - & - & - & - & - & - & - & 0.00 & 0.00 & 0.00 & 0.99 \\
Have pleasure & - & - & - & - & 0.00 & 0.00 & 0.00 & 0.98 & 0.00 & 0.00 & 0.00 & 0.98 & 0.00 & 0.00 & 0.00 & 0.99 \\
Be ambitious & 0.00 & 0.00 & 0.00 & 0.96 & 0.00 & 0.00 & 0.00 & 0.95 & 1.00 & 0.20 & 0.33 & 0.96 & 1.00 & 0.03 & 0.07 & 0.94 \\
Have success & 0.71 & 1.00 & 0.83 & 0.96 & 0.38 & 0.50 & 0.43 & 0.79 & 0.64 & 0.58 & 0.61 & 0.91 & 0.77 & 0.32 & 0.45 & 0.86 \\
Be capable & 0.00 & 0.00 & 0.00 & 0.86 & 0.42 & 0.25 & 0.31 & 0.78 & 0.60 & 0.60 & 0.60 & 0.88 & 0.57 & 0.20 & 0.30 & 0.84 \\
Be intellectual & 0.00 & 0.00 & 0.00 & 0.94 & 0.75 & 0.23 & 0.35 & 0.89 & 0.50 & 0.50 & 0.50 & 0.98 & 0.65 & 0.20 & 0.30 & 0.86 \\
Be courageous & 0.00 & 0.00 & 0.00 & 0.98 & - & - & - & - & - & - & - & - & 0.00 & 0.00 & 0.00 & 1.00 \\
Have influence & 0.00 & 0.00 & 0.00 & 0.90 & 0.00 & 0.00 & 0.00 & 0.98 & - & - & - & - & 0.14 & 0.03 & 0.05 & 0.92 \\
Have the right to command & - & - & - & - & - & - & - & - & 0.00 & 0.00 & 0.00 & 0.99 & 0.00 & 0.00 & 0.00 & 0.93 \\
Have wealth & 1.00 & 1.00 & 1.00 & 1.00 & 0.35 & 0.58 & 0.44 & 0.72 & 0.30 & 1.00 & 0.46 & 0.93 & 0.39 & 0.53 & 0.45 & 0.92 \\
Have social recognition & 0.00 & 0.00 & 0.00 & 0.96 & - & - & - & - & 0.00 & 0.00 & 0.00 & 0.98 & 0.00 & 0.00 & 0.00 & 0.96 \\
Have a good reputation & 0.00 & 0.00 & 0.00 & 0.98 & 0.00 & 0.00 & 0.00 & 0.99 & 0.00 & 0.00 & 0.00 & 0.97 & 0.00 & 0.00 & 0.00 & 0.99 \\
Have a sense of belonging & 0.00 & 0.00 & 0.00 & 0.84 & 0.00 & 0.00 & 0.00 & 0.96 & 0.00 & 0.00 & 0.00 & 0.98 & 0.56 & 0.49 & 0.52 & 0.92 \\
Have good health & 0.00 & 0.00 & 0.00 & 0.92 & 0.00 & 0.00 & 0.00 & 0.95 & 0.88 & 0.58 & 0.70 & 0.94 & 0.80 & 0.81 & 0.81 & 0.93 \\
Have no debts & - & - & - & - & 0.00 & 0.00 & 0.00 & 0.95 & 0.50 & 0.50 & 0.50 & 0.98 & 0.68 & 0.41 & 0.51 & 0.94 \\
Be neat and tidy & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
Have a comfortable life & 0.38 & 0.75 & 0.50 & 0.88 & 0.43 & 0.35 & 0.38 & 0.71 & 0.56 & 0.26 & 0.36 & 0.82 & 0.52 & 0.61 & 0.56 & 0.81 \\
Have a safe country & 0.29 & 0.62 & 0.40 & 0.70 & 0.40 & 0.67 & 0.50 & 0.96 & 0.62 & 0.56 & 0.59 & 0.86 & 0.43 & 0.24 & 0.31 & 0.92 \\
Have a stable society & 0.50 & 0.81 & 0.62 & 0.58 & 0.53 & 0.53 & 0.53 & 0.72 & 0.37 & 0.41 & 0.39 & 0.78 & 0.55 & 0.36 & 0.44 & 0.81 \\
Be respecting traditions & 0.00 & 0.00 & 0.00 & 0.96 & - & - & - & - & 0.25 & 0.50 & 0.33 & 0.96 & 0.77 & 0.18 & 0.29 & 0.90 \\
Be holding religious faith & - & - & - & - & - & - & - & - & 1.00 & 0.80 & 0.89 & 0.99 & 0.46 & 0.13 & 0.21 & 0.91 \\
Be compliant & 0.00 & 0.00 & 0.00 & 0.84 & 0.29 & 0.29 & 0.29 & 0.90 & 0.20 & 0.20 & 0.20 & 0.84 & 0.75 & 0.22 & 0.34 & 0.88 \\
Be self-disciplined & - & - & - & - & 0.00 & 0.00 & 0.00 & 0.97 & 0.00 & 0.00 & 0.00 & 0.99 & 0.00 & 0.00 & 0.00 & 0.97 \\
Be behaving properly & 0.50 & 0.25 & 0.33 & 0.84 & 0.00 & 0.00 & 0.00 & 0.82 & 0.41 & 0.39 & 0.40 & 0.79 & 0.25 & 0.09 & 0.14 & 0.87 \\
Be polite & - & - & - & - & 0.00 & 0.00 & 0.00 & 0.99 & 0.00 & 0.00 & 0.00 & 0.97 & 1.00 & 0.25 & 0.40 & 0.99 \\
Be honoring elders & - & - & - & - & - & - & - & - & - & - & - & - & 0.00 & 0.00 & 0.00 & 0.99 \\
Be humble & 0.00 & 0.00 & 0.00 & 0.92 & 0.00 & 0.00 & 0.00 & 0.98 & 0.00 & 0.00 & 0.00 & 0.99 & 0.00 & 0.00 & 0.00 & 0.98 \\
Have life accepted as is & 0.00 & 0.00 & 0.00 & 0.96 & 0.00 & 0.00 & 0.00 & 0.95 & 0.50 & 0.25 & 0.33 & 0.96 & 0.50 & 0.08 & 0.14 & 0.93 \\
Be helpful & 0.25 & 0.33 & 0.29 & 0.90 & 0.20 & 0.33 & 0.25 & 0.94 & 0.33 & 0.25 & 0.29 & 0.95 & 0.38 & 0.46 & 0.42 & 0.75 \\
Be honest & 0.00 & 0.00 & 0.00 & 0.94 & 0.00 & 0.00 & 0.00 & 0.99 & 0.00 & 0.00 & 0.00 & 0.97 & 1.00 & 0.05 & 0.09 & 0.96 \\
Be forgiving & - & - & - & - & - & - & - & - & 0.00 & 0.00 & 0.00 & 0.99 & 0.50 & 0.33 & 0.40 & 0.99 \\
Have the own family secured & - & - & - & - & 1.00 & 0.22 & 0.36 & 0.93 & 1.00 & 0.33 & 0.50 & 0.98 & 0.64 & 0.31 & 0.42 & 0.91 \\
Be loving & 0.00 & 0.00 & 0.00 & 0.98 & 1.00 & 0.50 & 0.67 & 0.99 & 0.00 & 0.00 & 0.00 & 0.96 & 0.20 & 0.14 & 0.17 & 0.96 \\
Be responsible & 0.00 & 0.00 & 0.00 & 0.92 & 0.00 & 0.00 & 0.00 & 0.94 & 0.50 & 0.09 & 0.15 & 0.89 & 0.44 & 0.13 & 0.20 & 0.87 \\
Have loyalty towards friends & - & - & - & - & - & - & - & - & - & - & - & - & 0.00 & 0.00 & 0.00 & 0.99 \\
Have equality & 0.53 & 0.67 & 0.59 & 0.78 & 0.25 & 0.33 & 0.29 & 0.85 & 0.80 & 0.40 & 0.53 & 0.86 & 0.31 & 0.34 & 0.33 & 0.76 \\
Be just & 0.11 & 0.67 & 0.18 & 0.64 & 0.35 & 0.44 & 0.39 & 0.75 & 0.55 & 0.69 & 0.61 & 0.86 & 0.56 & 0.50 & 0.53 & 0.79 \\
Have a world at peace & 0.57 & 0.31 & 0.40 & 0.76 & - & - & - & - & 0.67 & 0.50 & 0.57 & 0.97 & 0.67 & 0.12 & 0.20 & 0.97 \\
Be protecting the environment & - & - & - & - & 0.67 & 0.25 & 0.36 & 0.93 & 1.00 & 1.00 & 1.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.99 \\
Have harmony with nature & - & - & - & - & 0.67 & 0.40 & 0.50 & 0.96 & 0.50 & 0.20 & 0.29 & 0.95 & 0.78 & 0.22 & 0.34 & 0.95 \\
Have a world of beauty & - & - & - & - & - & - & - & - & - & - & - & - & 0.00 & 0.00 & 0.00 & 1.00 \\
Be broadminded & 0.00 & 0.00 & 0.00 & 0.88 & 0.00 & 0.00 & 0.00 & 0.97 & 0.00 & 0.00 & 0.00 & 0.91 & 0.23 & 0.12 & 0.16 & 0.83 \\
Have the wisdom to accept others & 0.00 & 0.00 & 0.00 & 0.98 & 0.00 & 0.00 & 0.00 & 0.99 & - & - & - & - & 0.17 & 0.03 & 0.06 & 0.93 \\
Be logical & 0.00 & 0.00 & 0.00 & 0.98 & 0.00 & 0.00 & 0.00 & 0.87 & 0.00 & 0.00 & 0.00 & 0.91 & 0.55 & 0.11 & 0.18 & 0.89 \\
Have an objective view & 0.00 & 0.00 & 0.00 & 0.82 & 0.00 & 0.00 & 0.00 & 0.79 & 0.00 & 0.00 & 0.00 & 0.83 & 0.39 & 0.31 & 0.35 & 0.83 \\
\bottomrule
\end{tabular}
\caption{Only testing}
\label{table-bert-label-scores}
\end{table*}5393
